DROP: Dimensionality Reduction Optimization for Time Series

Dimensionality reduction is a critical step in scaling machine learning pipelines. Principal component analysis (PCA) is a standard tool for dimensionality reduction, but performing PCA over a full dataset can be prohibitively expensive. As a result, theoretical work has studied the effectiveness of iterative, stochastic PCA methods that operate over data samples. However, termination conditions for stochastic PCA either execute for a predetermined number of iterations, or until convergence of the solution, frequently sampling too many or too few datapoints for end-to-end runtime improvements. We show how accounting for downstream analytics operations during DR via PCA allows stochastic methods to efficiently terminate after operating over small (e.g., 1%) subsamples of input data, reducing whole workload runtime. Leveraging this, we propose DROP, a DR optimizer that enables speedups of up to 5x over Singular-Value-Decomposition-based PCA techniques, and exceeds conventional approaches like FFT and PAA by up to 16x in end-to-end workloads.

==> abstract.tex <==
\section*{abstract}
Dimensionality reduction is a critical step in scaling machine learning pipelines. Principal component analysis (PCA) is a standard tool for dimensionality reduction, but performing PCA over a full dataset can be prohibitively expensive. 
As a result, theoretical work has studied the effectiveness of iterative, stochastic PCA methods that operate over data samples. 
However, termination conditions for stochastic PCA either execute for a predetermined number of iterations, or until convergence of the solution, frequently sampling too many or too few datapoints for end-to-end runtime improvements. We show how accounting for downstream analytics operations during DR via PCA allows stochastic methods to efficiently terminate after operating over small (e.g., 1\%) subsamples of input data, reducing whole workload runtime. 
Leveraging this, we propose DROP, a DR optimizer that enables speedups of up to \red{$5\times$} over \red{Singular-Value-Decomposition-based} PCA techniques, and exceeds conventional approaches like FFT and PAA by up to \red{$16\times$} in end-to-end workloads.




%This enables end-to-end optimization over both dimensionality reduction and analytics tasks.
%By combining techniques spanning progressive sampling, approximate query processing, and cost-based optimization, we propose a dimensionality reduction optimizer that enables speedups of up to \red{$5\times$} over \red{Singular-Value-Decomposition-based} PCA techniques, and achieves parity with or exceeds conventional approaches like FFT and PAA by up to \red{$16\times$} in end-to-end workloads.

%As time series analytics workloads grow, we see an increase in time series tools and DB stuff to enable more efficient TS analytics routines. 
%In order to facilitate this, indexing of time series is important---and DR plays a critical step in this.





%DROP uses the key insight that structured data such as time series can be sufficiently characterized by a small subset of data, which permits aggressive sampling during dimensionality reduction.  
%Sampling allows DROP to uncover high quality low-dimensional bases in runtime proportional to the dataset's intrinsic dimensionality---\textit{independent} of the actual dataset size.
%Additionally, DROP uses online progress estimation to predict DROP and downstream runtime costs, enabling a trade-off between degree of dimensionality reduction and pipeline runtime, and obviating the need for the intrinsic data dimension to be specified by the user. 
%At a high level, DROP progressively samples its input, computes a candidate transformation, and terminates once it finds a low dimensional representation of suitable size and quality quickly enough to not bottleneck downstream tasks. DROP provides speedups of up to $50\times$ over the na\"ive, SVD-based approach and $33\times$  in end-to-end analytics pipelines.
%A dataset's intrinsic dimensionality is also typically unknown a priori (i.e., to what extent a dataset can be compressed), a necessary parameter for dimensionality reduction via PCA.
%Further, based on downstream analytics tasks, it may be crucial to quickly return a result even if it is of dimension higher than the intrinsic dimension, but sufficient for the task at hand.
%To address these challenges, we present DROP, a new dynamic optimizer for high-dimensional analytics pipelines that efficiently computes high quality results (low-dimensional bases) via approximate PCA, without PCA's expensive runtime.
%dimensionality reduction optimizer that efficiently performs PCA in high-dimensional analytics pipelines.
%new dynamic optimizer that efficiently computes high quality results (i.e., low-dimensional basis) without the expensive runtime of PCA
%DROP reduces the cost of PCA over structured datasets, and automatically identifies a low dimensional data representation by taking the runtime of downstream analytics tasks into consideration.




%DROP enables downstream-operation-aware optimization via online progress estimation, trading-off degree of dimensionality reduction with the combined runtime of DROP and downstream analytics tasks. 

%In this paper, we revisit a now-classic study of time series dimensionality reduction operators and find that for a given quality constraint, Principal Component Analysis (PCA) uncovers representations that are over $2\times$ smaller than those obtained via alternative techniques favored in the time series literature. 


==> appendices.tex <==
\appendix
\section*{APPENDIX}

\section{Augmented Results}


In this section, we provide additional information to augment results provided in our time series case study. 
Table~\ref{tab:sample} displays the proportion of data required to attain a given $TLB$ when using a PCA transformation where output dimension is equal to input dimension. Table~\ref{tab:kneeded} illustrates the output dimension required for each algorithm (PAA, FFT, and PCA) to attain a target $TLB$. 
Table~\ref{tab:runtime-comparison} illustrates the different running times of each algorithm (PAA, FFT, and PCA), and how sampling using the proportion from Table~\ref{tab:sample} for $TLB=0.99$ can help bridge the time gap between SVD and other techniques. 
%Finally, we provide all of the remaining lesion studies for the UCR dataset.


\begin{table}[]
\centering
\caption{Normalized lower dimension for target $TLB$ across DR techniques. PCA admits lower dimension for most UCR time series datasets.}
\label{tab:kneeded}
\scriptsize
\begin{tabular}{|l|r|r|r|r|r|r|}
\hline
                                  & \multicolumn{3}{c|}{\textbf{TLB:0.75}}     & \multicolumn{3}{c|}{\textbf{TLB:0.99}}     \\ \hline
\textbf{Dataset (dimension)} & \textit{PAA} & \textit{FFT} & \textit{PCA} & \textit{PAA} & \textit{FFT} & \textit{PCA} \\ \hline
ElectricDevices (96)              & 0.126        & 0.094        & 0.032        & 0.594        & 0.212        & 0.164        \\ \hline
FordA (500)                       & 0.138        & 0.098        & 0.038        & 0.636        & 0.214        & 0.17         \\ \hline
FordB (500)                       & 0.018        & 0.029        & 0.009        & 0.290        & 0.177        & 0.035        \\ \hline
MALLAT (1024)                     & 0.084        & 0.068        & 0.057        & 0.898        & 0.837        & 0.522        \\ \hline
Phoneme (1024)                    & 0.004        & 0.026        & 0.001        & 0.049        & 0.035        & 0.034        \\ \hline
StarLightCurves (1024)            & 0.015        & 0.028        & 0.019        & 0.037        & 0.086        & 0.062        \\ \hline
UWGLAll (945)                     & 0.078        & 0.065        & 0.026        & 0.822        & 0.736        & 0.322        \\ \hline
wafer (152)                       & 0.014        & 0.030        & 0.007        & 0.103        & 0.049        & 0.037        \\ \hline
yoga (426)                        & 0.375        & 0.375        & 0.281        & 0.812        & 0.822        & 0.770        \\ \hline

\end{tabular}
\end{table}



\begin{table}[]
\centering
\caption{Runtime (in ms) of 3 DR techniques. PCA is slowest, and can be over $56\times$ slower than PAA. Running SVD over a sample can bridge this gap.}
\label{tab:runtime-comparison}
\scriptsize
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Dataset}        & \textbf{PAA ($\times$SVD)} & \textbf{FFT} & \textbf{SVD} & \textbf{Sampling} \\ \hline
ElectricDevices         & 3 (9.8$\times$)            & 18           & 33           & 6                 \\ \hline
FordA                   & 7 (19$\times$)             & 38           & 137          & 8                 \\ \hline
FordB                   & 7 (18$\times$)             & 32           & 121          & 7                 \\ \hline
MALLAT                  & 7 (37.6$\times$)           & 35           & 278          & 5                 \\ \hline
Phoneme                 & 5 (56.2$\times$)           & 29           & 281          & 164               \\ \hline
StarLightCurves         & 19 (24.1$\times$)          & 120          & 457          & 5                 \\ \hline
UWGLAll & 7 (43.5$\times$)           & 56           & 287          & 8                 \\ \hline
Wafer                   & 4 (6.1$\times$)            & 13           & 22           & 5                 \\ \hline
Yoga                    & 4 (21.2$\times$)           & 29           & 81           & 8                 \\ \hline
\end{tabular}
\end{table}



\begin{table}[]
\centering
\scriptsize
\caption{A small proportion of data is needed to obtain a $TLB$-preserving transform with full PCA (output = input dimension).}

\begin{tabular}{|l|r|r|r|}
\hline
                               & \multicolumn{3}{c|}{\textit{\textbf{TLB}}}    \\ \hline
\textbf{Dataset (number of datapoints)}               & \textbf{0.75} & \textbf{0.90} & \textbf{0.99} \\ \hline
ElectricDevices (16637)               & 0.0026        & 0.0043        & 0.0088        \\ \hline
FordA   (4921)                       & 0.0054        & 0.0114        & 0.0198        \\ \hline
FordB   (4446)                       & 0.008         & 0.0146        & 0.0248        \\ \hline
MALLAT  (2400)                       & 0.0031        & 0.009         & 0.0197        \\ \hline
Phoneme   (2110)                     & 0.0547        & 0.1346        & 0.3875        \\ \hline
StarLightCurves (9236)               & 0.001         & 0.0011        & 0.0039        \\ \hline
UWGLAll  (4478)       & 0.0025        & 0.0056        & 0.024         \\ \hline
wafer  (7164)                        & 0.001         & 0.0032        & 0.0097        \\ \hline
yoga  (3300)                         & 0.0017        & 0.0028        & 0.0096        \\ \hline
\end{tabular}
\label{tab:sample}
\end{table}






\begin{comment}
\begin{table}[b]
\centering
\scriptsize
\caption{End-to-End runtime comparison of DROP and baseline techniques with k-NN retrieval task, in ms}
\label{tab:eefull}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\textbf{Dataset}       & \textbf{No DR} & \textbf{SVD} & \textbf{SVD-Halko} & \textbf{Oracle} & \textbf{DROP} \\ \hline
ChlorineConcentration  & 458   & 4054  & 424   & 207   & 178   \\ \hline
CinC                   & 1809  & 3068  & 5738  & 884   & 894   \\ \hline
ECG5000                & 1855  & 5689  & 561   & 362   & 482   \\ \hline
ElectricDevices        & 38222 & 83302 & 28433 & 27260 & 30701 \\ \hline
FordA                  & 21906 & 10546 & 5300  & 4270  & 4286  \\ \hline
FordB                  & 18271 & 8984  & 4917  & 3773  & 3792  \\ \hline
HandOutlines           & 5160  & 5620  & 9479  & 2832  & 2678  \\ \hline
InlineSkate            & 579   & 1420  & 2081  & 548   & 704   \\ \hline
InsectWingbeatSound    & 805   & 977   & 425   & 200   & 212   \\ \hline
MALLAT                 & 2593  & 2895  & 3870  & 643   & 450   \\ \hline
NonInvasiveFatalECG    & 5157  & 5229  & 3235  & 944   & 1043  \\ \hline
Phoneme                & 8490  & 6710  & 7687  & 7534  & 10446 \\ \hline
StarLightCurves        & 32024 & 35129 & 11429 & 1079  & 1238  \\ \hline
Two                    & 5728  & 8916  & 2849  & 2860  & 3335  \\ \hline
UWaveGestureLibraryAll & 25825 & 8147  & 5509  & 1298  & 1355  \\ \hline
uWaveGestureLibrary    & 4734  & 5669  & 1067  & 402   & 310   \\ \hline
wafer                  & 1536  & 12911 & 749   & 403   & 403   \\ \hline
yoga                   & 1199  & 2943  & 1029  & 174   & 153   \\ \hline
\end{tabular}
\end{table}


\begin{table}[b]
\centering
\scriptsize
\caption{Raw accuracy in k-NN retrieval task}
\label{tab:knn}
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Dataset}   & \textbf{SVD} & \textbf{SVD-Halko} & \textbf{Oracle} & \textbf{DROP} \\ \hline
ChlorineConcentration  & 0.893        & 0.886              & 0.906           & 0.903         \\ \hline
CinC                   & 0.894        & 0.892              & 0.899           & 0.929         \\ \hline
ECG5000                & 0.855        & 0.855              & 0.856           & 0.874         \\ \hline
ElectricDevices        & 0.877        & 0.875              & 0.866           & 0.888         \\ \hline
FordA                  & 0.892        & 0.878              & 0.884           & 0.9           \\ \hline
FordB                  & 0.875        & 0.875              & 0.871           & 0.874         \\ \hline
HandOutlines           & 0.908        & 0.901              & 0.907           & 0.92          \\ \hline
InlineSkate            & 0.832        & 0.818              & 0.803           & 0.805         \\ \hline
InsectWingbeatSound    & 0.815        & 0.815              & 0.811           & 0.848         \\ \hline
MALLAT                 & 0.83         & 0.83               & 0.876           & 0.892         \\ \hline
NonInvasiveFatalECG    & 0.82         & 0.822              & 0.836           & 0.827         \\ \hline
Phoneme                & 0.848        & 0.852              & 0.68            & 0.678         \\ \hline
StarLightCurves        & 0.615        & 0.648              & 0.653           & 0.651         \\ \hline
Two                    & 0.899        & 0.903              & 0.901           & 0.902         \\ \hline
UWaveGestureLibraryAll & 0.846        & 0.853              & 0.856           & 0.883         \\ \hline
uWaveGestureLibrary    & 0.797        & 0.797              & 0.808           & 0.838         \\ \hline
wafer                  & 0.808        & 0.818              & 0.833           & 0.888         \\ \hline
yoga                   & 0.791        & 0.791              & 0.797           & 0.818         \\ \hline
\end{tabular}
\end{table}


\end{comment}


\begin{comment}
\begin{table*}[]
\centering
\scriptsize
\caption{Output dimension required for target $TLB$ across dimensionality reduction technique (right 9 data columns), and proportion of data required to obtain a $TLB$-preserving PCA transformation with output dimension = input dimension (final 3 columns)}
\label{tab:bigtab}
\begin{tabular}{| c ||ccc|ccc|ccc||cc||ccc|}
\hline

 & \multicolumn{3}{c|}{\textbf{TLB: 0.75}} & \multicolumn{3}{c|}{\textbf{TLB: 0.90}} & \multicolumn{3}{c||}{\textbf{TLB: 0.99}} &  &  & \multicolumn{3}{c|}{\textbf{TLB}}  \\

\textbf{Dataset} & \textit{PAA }     & \textit{FFT}     & \textit{PCA}     & \textit{PAA}      & \textit{FFT}      & \textit{PCA}     & \textit{PAA}      & \textit{FFT}     &\textit{PCA}     &  &  & \textit{0.75}   & \textit{0.90 }  & \textit{0.99}   \\
\hline
50words                        & 9        & 9        & 7       & 18       & 14       & 10      & 62       & 28       & 25      &  &  & 0.0106 & 0.0185 & 0.0391 \\
Adiac                          & 7        & 8        & 4       & 15       & 13       & 6       & 69       & 34       & 20      &  &  & 0.0077 & 0.0145 & 0.0484 \\
ArrowHead                      & 9        & 9        & 4       & 16       & 13       & 8       & 73       & 33       & 26      &  &  & 0.0285 & 0.0626 & 0.2907 \\
Beef                           & 7        & 15       & 2       & 20       & 18       & 3       & 89       & 48       & 7       &  &  & 0.0494 & 0.0898 & 0.19   \\
BeetleFly                      & 16       & 16       & 6       & 28       & 21       & 12      & 99       & 34       & 22      &  &  & 0.3073 & 0.4449 & 0.7979 \\
BirdChicken                    & 8        & 14       & 3       & 14       & 17       & 6       & 48       & 20       & 15      &  &  & 0.156  & 0.2357 & 0.5437 \\
Car                            & 7        & 16       & 2       & 15       & 19       & 6       & 70       & 37       & 24      &  &  & 0.0428 & 0.0979 & 0.3719 \\
CBF                            & 15       & 13       & 7       & 61       & 57       & 45      & 114      & 114      & 107     &  &  & 0.0273 & 0.0775 & 0.1407 \\
ChlorineConcentration          & 46       & 34       & 2       & 93       & 81       & 5       & 153      & 153      & 30      &  &  & 0.001  & 0.0029 & 0.014  \\
CinC                           & 29       & 44       & 26      & 58       & 53       & 40      & 241      & 107      & 48      &  &  & 0.007  & 0.0157 & 0.0391 \\
Coffee                         & 14       & 17       & 3       & 46       & 37       & 6       & 225      & 158      & 38      &  &  & 0.1224 & 0.2715 & 0.8632 \\
Computers                      & 21       & 24       & 16      & 94       & 66       & 44      & 636      & 614      & 192     &  &  & 0.0596 & 0.1889 & 0.6818 \\
Cricket                        & 14       & 14       & 9       & 47       & 35       & 21      & 248      & 202      & 113     &  &  & 0.0198 & 0.0574 & 0.2488 \\
DiatomSizeReduction            & 7        & 11       & 7       & 11       & 13       & 10      & 87       & 55       & 21      &  &  & 0.015  & 0.0282 & 0.176  \\
DistalPhalanxOutlineAgeGroup   & 12       & 12       & 2       & 27       & 17       & 6       & 66       & 60       & 36      &  &  & 0.0094 & 0.0241 & 0.0987 \\
DistalPhalanxOutlineCorrect    & 12       & 12       & 2       & 26       & 16       & 7       & 66       & 57       & 32      &  &  & 0.006  & 0.0168 & 0.0642 \\
DistalPhalanxTW                & 12       & 12       & 2       & 27       & 16       & 6       & 66       & 60       & 34      &  &  & 0.0097 & 0.0236 & 0.098  \\
Earthquakes                    & 276      & 269      & 103     & 410      & 400      & 190     & 491      & 490      & 340     &  &  & 0.3733 & 0.6052 & 0.8988 \\
ECG200                         & 8        & 7        & 3       & 29       & 22       & 6       & 72       & 56       & 41      &  &  & 0.0288 & 0.0942 & 0.3287 \\
ECG5000                        & 14       & 14       & 3       & 30       & 24       & 7       & 115      & 88       & 31      &  &  & 0.001  & 0.0025 & 0.0132 \\
ECGFiveDays                    & 31       & 28       & 2       & 53       & 40       & 5       & 111      & 65       & 13      &  &  & 0.0073 & 0.0114 & 0.0275 \\
ElectricDevices                & 36       & 36       & 27      & 62       & 57       & 49      & 78       & 79       & 74      &  &  & 0.0026 & 0.0043 & 0.0088 \\
FaceAll                        & 28       & 24       & 8       & 50       & 35       & 20      & 110      & 81       & 48      &  &  & 0.0078 & 0.0171 & 0.0355 \\
FaceFour                       & 36       & 31       & 5       & 67       & 43       & 12      & 277      & 228      & 61      &  &  & 0.1143 & 0.2727 & 0.7708 \\
FacesUCR                       & 28       & 24       & 9       & 48       & 34       & 22      & 109      & 53       & 49      &  &  & 0.0077 & 0.0169 & 0.0355 \\
FISH                           & 10       & 15       & 5       & 20       & 18       & 11      & 91       & 37       & 28      &  &  & 0.0181 & 0.0433 & 0.1587 \\
FordA                          & 63       & 47       & 16      & 98       & 61       & 35      & 297      & 106      & 82      &  &  & 0.0054 & 0.0114 & 0.0198 \\
FordB                          & 69       & 49       & 19      & 102      & 65       & 39      & 318      & 107      & 85      &  &  & 0.008  & 0.0146 & 0.0248 \\
Gun                            & 5        & 6        & 3       & 11       & 9        & 5       & 56       & 24       & 14      &  &  & 0.0282 & 0.0477 & 0.134  \\
Ham                            & 34       & 32       & 7       & 73       & 58       & 18      & 261      & 114      & 61      &  &  & 0.0811 & 0.1558 & 0.4486 \\
HandOutlines                   & 11       & 70       & 10      & 25       & 83       & 32      & 93       & 91       & 46      &  &  & 0.0045 & 0.0091 & 0.0372 \\
Haptics                        & 10       & 29       & 6       & 19       & 35       & 14      & 173      & 81       & 32      &  &  & 0.017  & 0.0394 & 0.1234 \\
Herring                        & 10       & 15       & 3       & 25       & 18       & 8       & 111      & 63       & 39      &  &  & 0.0599 & 0.1447 & 0.4878 \\
InlineSkate                    & 7        & 49       & 7       & 15       & 58       & 17      & 55       & 63       & 22      &  &  & 0.0085 & 0.0162 & 0.0388 \\
InsectWingbeatSound            & 15       & 14       & 7       & 28       & 22       & 13      & 100      & 42       & 33      &  &  & 0.0048 & 0.0119 & 0.0255 \\
ItalyPowerDemand               & 6        & 6        & 2       & 11       & 10       & 5       & 19       & 17       & 15      &  &  & 0.0068 & 0.01   & 0.0198 \\
LargeKitchenAppliances         & 59       & 49       & 36      & 165      & 125      & 89      & 624      & 545      & 284     &  &  & 0.0987 & 0.2373 & 0.6068 \\
Lighting2                      & 41       & 34       & 9       & 152      & 149      & 28      & 557      & 490      & 82      &  &  & 0.186  & 0.4505 & 0.9132 \\
Lighting7                      & 31       & 27       & 9       & 126      & 118      & 26      & 280      & 269      & 81      &  &  & 0.1439 & 0.3534 & 0.9022 \\
MALLAT                         & 19       & 30       & 10      & 46       & 36       & 26      & 297      & 182      & 36      &  &  & 0.0031 & 0.009  & 0.0197 \\
Meat                           & 13       & 14       & 2       & 32       & 24       & 4       & 218      & 213      & 23      &  &  & 0.0398 & 0.0528 & 0.3494 \\
MedicalImages                  & 12       & 10       & 3       & 20       & 17       & 7       & 66       & 34       & 17      &  &  & 0.007  & 0.0103 & 0.0256 \\
MiddlePhalanxOutlineAgeGroup   & 12       & 12       & 2       & 27       & 16       & 4       & 66       & 60       & 31      &  &  & 0.0096 & 0.0191 & 0.0939 \\
MiddlePhalanxOutlineCorrect    & 12       & 12       & 2       & 27       & 16       & 5       & 66       & 58       & 30      &  &  & 0.0065 & 0.0127 & 0.0548 \\
MiddlePhalanxTW                & 12       & 12       & 2       & 27       & 16       & 5       & 66       & 60       & 32      &  &  & 0.0089 & 0.0206 & 0.0916 \\
MoteStrain                     & 12       & 11       & 7       & 39       & 37       & 26      & 76       & 75       & 63      &  &  & 0.0148 & 0.0323 & 0.0838 \\
NonInvasiveFatalECG            & 16       & 22       & 3       & 42       & 31       & 18      & 201      & 121      & 82      &  &  & 0.0021 & 0.0043 & 0.0375 \\
OliveOil                       & 33       & 25       & 2       & 61       & 51       & 5       & 375      & 213      & 23      &  &  & 0.0936 & 0.1727 & 0.6366 \\
OSULeaf                        & 11       & 13       & 9       & 20       & 16       & 14      & 73       & 30       & 29      &  &  & 0.0258 & 0.0435 & 0.1104 \\
PhalangesOutlinesCorrect       & 11       & 12       & 2       & 26       & 16       & 5       & 65       & 56       & 28      &  &  & 0.0023 & 0.0046 & 0.0187 \\
Phoneme                        & 87       & 70       & 59      & 268      & 201      & 160     & 920      & 858      & 535     &  &  & 0.0547 & 0.1346 & 0.3875 \\
Plane                          & 12       & 11       & 3       & 22       & 14       & 6       & 76       & 39       & 21      &  &  & 0.0285 & 0.0683 & 0.2068 \\
ProximalPhalanxOutlineAgeGroup & 12       & 12       & 2       & 26       & 18       & 4       & 65       & 58       & 28      &  &  & 0.0068 & 0.0171 & 0.0825 \\
ProximalPhalanxOutlineCorrect  & 12       & 12       & 2       & 27       & 18       & 5       & 66       & 58       & 28      &  &  & 0.0046 & 0.0134 & 0.0512 \\
ProximalPhalanxTW              & 12       & 12       & 2       & 26       & 18       & 5       & 65       & 59       & 28      &  &  & 0.0052 & 0.0153 & 0.0831 \\
RefrigerationDevices           & 94       & 76       & 60      & 222      & 154      & 121     & 645      & 586      & 316     &  &  & 0.1414 & 0.2777 & 0.6696 \\
ScreenType                     & 18       & 24       & 20      & 70       & 55       & 40      & 614      & 614      & 207     &  &  & 0.0324 & 0.1087 & 0.5341 \\
ShapeletSim                    & 275      & 272      & 62      & 410      & 402      & 111     & 491      & 490      & 180     &  &  & 0.497  & 0.7498 & 0.969  \\
ShapesAll                      & 7        & 14       & 7       & 14       & 17       & 14      & 49       & 25       & 20      &  &  & 0.0048 & 0.0137 & 0.0278 \\
SmallKitchenAppliances         & 259      & 235      & 104     & 497      & 423      & 204     & 698      & 678      & 398     &  &  & 0.2489 & 0.422  & 0.7194 \\
SonyAIBORobotSurface           & 15       & 14       & 5       & 28       & 21       & 13      & 56       & 43       & 38      &  &  & 0.0211 & 0.0442 & 0.0969 \\
SonyAIBORobotSurfaceII         & 18       & 18       & 6       & 30       & 24       & 13      & 57       & 45       & 39      &  &  & 0.0143 & 0.0272 & 0.0708 \\
StarLightCurves                & 5        & 27       & 2       & 14       & 33       & 21      & 51       & 36       & 35      &  &  & 0.001  & 0.0011 & 0.0039 \\
Strawberry                     & 10       & 11       & 2       & 24       & 21       & 6       & 98       & 41       & 13      &  &  & 0.005  & 0.0086 & 0.0225 \\
SwedishLeaf                    & 9        & 9        & 5       & 19       & 14       & 10      & 71       & 37       & 32      &  &  & 0.0083 & 0.0178 & 0.0727 \\
Symbols                        & 7        & 11       & 6       & 12       & 13       & 11      & 46       & 26       & 14      &  &  & 0.0071 & 0.0096 & 0.0246 \\
synthetic                      & 14       & 14       & 7       & 37       & 38       & 28      & 58       & 59       & 54      &  &  & 0.0281 & 0.0642 & 0.0964 \\
ToeSegmentation1               & 12       & 10       & 8       & 24       & 19       & 16      & 116      & 49       & 43      &  &  & 0.0548 & 0.0992 & 0.2988 \\
ToeSegmentation2               & 10       & 13       & 6       & 21       & 20       & 13      & 101      & 49       & 34      &  &  & 0.0718 & 0.144  & 0.3784 \\
Trace                          & 6        & 9        & 2       & 18       & 17       & 7       & 120      & 69       & 31      &  &  & 0.0222 & 0.0555 & 0.3752 \\
TwoLeadECG                     & 12       & 9        & 2       & 25       & 19       & 4       & 70       & 51       & 14      &  &  & 0.0045 & 0.0081 & 0.0259 \\
Two                            & 13       & 11       & 7       & 34       & 24       & 20      & 108      & 102      & 98      &  &  & 0.0038 & 0.0097 & 0.0259 \\
UWaveGestureLibraryAll         & 15       & 27       & 18      & 35       & 32       & 28      & 151      & 82       & 59      &  &  & 0.0025 & 0.0056 & 0.024  \\
uWaveGestureLibrary            & 4        & 10       & 5       & 10       & 11       & 10      & 43       & 27       & 20      &  &  & 0.0017 & 0.0024 & 0.0081 \\
wafer                          & 12       & 10       & 4       & 37       & 29       & 11      & 125      & 112      & 49      &  &  & 0.001  & 0.0032 & 0.0097 \\
Wine                           & 10       & 9        & 2       & 27       & 20       & 3       & 104      & 58       & 9       &  &  & 0.031  & 0.0477 & 0.1745 \\
WordsSynonyms                  & 9        & 9        & 7       & 17       & 14       & 10      & 62       & 31       & 25      &  &  & 0.0094 & 0.0196 & 0.0389 \\
Worms                          & 9        & 26       & 8       & 26       & 30       & 17      & 123      & 62       & 41      &  &  & 0.0661 & 0.109  & 0.3177 \\
WormsTwoClass                  & 10       & 26       & 8       & 25       & 30       & 17      & 124      & 61       & 42      &  &  & 0.0575 & 0.1193 & 0.3289 \\
yoga                           & 6        & 13       & 3       & 11       & 15       & 11      & 44       & 21       & 16      &  &  & 0.0017 & 0.0028 & 0.0096 \\
\hline
\end{tabular}
\end{table*}
\end{comment}


\begin{comment}
\begin{table}[H]
\centering
\scriptsize
\caption{Proportion of data required to obtain a $TLB$-preserving transformation with full PCA (i.e., output dimension = input dimension)}

\begin{tabular}{|l|c|c|c|}
\hline
                               & \multicolumn{3}{c|}{\textit{\textbf{TLB}}}    \\ \hline
\textbf{Dataset}               & \textbf{0.75} & \textbf{0.90} & \textbf{0.99} \\ \hline
50words                        & 0.0106        & 0.0185        & 0.0391        \\ \hline
Adiac                          & 0.0077        & 0.0145        & 0.0484        \\ \hline
ArrowHead                      & 0.0285        & 0.0626        & 0.2907        \\ \hline
Beef                           & 0.0494        & 0.0898        & 0.19          \\ \hline
BeetleFly                      & 0.3073        & 0.4449        & 0.7979        \\ \hline
BirdChicken                    & 0.156         & 0.2357        & 0.5437        \\ \hline
Car                            & 0.0428        & 0.0979        & 0.3719        \\ \hline
CBF                            & 0.0273        & 0.0775        & 0.1407        \\ \hline
ChlorineConcentration          & 0.001         & 0.0029        & 0.014         \\ \hline
CinC                           & 0.007         & 0.0157        & 0.0391        \\ \hline
Coffee                         & 0.1224        & 0.2715        & 0.8632        \\ \hline
Computers                      & 0.0596        & 0.1889        & 0.6818        \\ \hline
Cricket                        & 0.0198        & 0.0574        & 0.2488        \\ \hline
DiatomSizeReduction            & 0.015         & 0.0282        & 0.176         \\ \hline
DistalPhalanxOutlineAgeGroup   & 0.0094        & 0.0241        & 0.0987        \\ \hline
DistalPhalanxOutlineCorrect    & 0.006         & 0.0168        & 0.0642        \\ \hline
DistalPhalanxTW                & 0.0097        & 0.0236        & 0.098         \\ \hline
Earthquakes                    & 0.3733        & 0.6052        & 0.8988        \\ \hline
ECG200                         & 0.0288        & 0.0942        & 0.3287        \\ \hline
ECG5000                        & 0.001         & 0.0025        & 0.0132        \\ \hline
ECGFiveDays                    & 0.0073        & 0.0114        & 0.0275        \\ \hline
ElectricDevices                & 0.0026        & 0.0043        & 0.0088        \\ \hline
FaceAll                        & 0.0078        & 0.0171        & 0.0355        \\ \hline
FaceFour                       & 0.1143        & 0.2727        & 0.7708        \\ \hline
FacesUCR                       & 0.0077        & 0.0169        & 0.0355        \\ \hline
FISH                           & 0.0181        & 0.0433        & 0.1587        \\ \hline
FordA                          & 0.0054        & 0.0114        & 0.0198        \\ \hline
FordB                          & 0.008         & 0.0146        & 0.0248        \\ \hline
Gun                            & 0.0282        & 0.0477        & 0.134         \\ \hline
Ham                            & 0.0811        & 0.1558        & 0.4486        \\ \hline
HandOutlines                   & 0.0045        & 0.0091        & 0.0372        \\ \hline
Haptics                        & 0.017         & 0.0394        & 0.1234        \\ \hline
Herring                        & 0.0599        & 0.1447        & 0.4878        \\ \hline
InlineSkate                    & 0.0085        & 0.0162        & 0.0388        \\ \hline
InsectWingbeatSound            & 0.0048        & 0.0119        & 0.0255        \\ \hline
ItalyPowerDemand               & 0.0068        & 0.01          & 0.0198        \\ \hline
LargeKitchenAppliances         & 0.0987        & 0.2373        & 0.6068        \\ \hline
Lighting2                      & 0.186         & 0.4505        & 0.9132        \\ \hline
Lighting7                      & 0.1439        & 0.3534        & 0.9022        \\ \hline
MALLAT                         & 0.0031        & 0.009         & 0.0197        \\ \hline
Meat                           & 0.0398        & 0.0528        & 0.3494        \\ \hline
MedicalImages                  & 0.007         & 0.0103        & 0.0256        \\ \hline
MiddlePhalanxOutlineAgeGroup   & 0.0096        & 0.0191        & 0.0939        \\ \hline
MiddlePhalanxOutlineCorrect    & 0.0065        & 0.0127        & 0.0548        \\ \hline
MiddlePhalanxTW                & 0.0089        & 0.0206        & 0.0916        \\ \hline
MoteStrain                     & 0.0148        & 0.0323        & 0.0838        \\ \hline
NonInvasiveFatalECG            & 0.0021        & 0.0043        & 0.0375        \\ \hline
OliveOil                       & 0.0936        & 0.1727        & 0.6366        \\ \hline
OSULeaf                        & 0.0258        & 0.0435        & 0.1104        \\ \hline
PhalangesOutlinesCorrect       & 0.0023        & 0.0046        & 0.0187        \\ \hline
Phoneme                        & 0.0547        & 0.1346        & 0.3875        \\ \hline
Plane                          & 0.0285        & 0.0683        & 0.2068        \\ \hline
ProximalPhalanxOutlineAgeGroup & 0.0068        & 0.0171        & 0.0825        \\ \hline
ProximalPhalanxOutlineCorrect  & 0.0046        & 0.0134        & 0.0512        \\ \hline
ProximalPhalanxTW              & 0.0052        & 0.0153        & 0.0831        \\ \hline
RefrigerationDevices           & 0.1414        & 0.2777        & 0.6696        \\ \hline
ScreenType                     & 0.0324        & 0.1087        & 0.5341        \\ \hline
ShapeletSim                    & 0.497         & 0.7498        & 0.969         \\ \hline
ShapesAll                      & 0.0048        & 0.0137        & 0.0278        \\ \hline
SmallKitchenAppliances         & 0.2489        & 0.422         & 0.7194        \\ \hline
SonyAIBORobotSurface           & 0.0211        & 0.0442        & 0.0969        \\ \hline
SonyAIBORobotSurfaceII         & 0.0143        & 0.0272        & 0.0708        \\ \hline
StarLightCurves                & 0.001         & 0.0011        & 0.0039        \\ \hline
Strawberry                     & 0.005         & 0.0086        & 0.0225        \\ \hline
SwedishLeaf                    & 0.0083        & 0.0178        & 0.0727        \\ \hline
Symbols                        & 0.0071        & 0.0096        & 0.0246        \\ \hline
synthetic                      & 0.0281        & 0.0642        & 0.0964        \\ \hline
ToeSegmentation1               & 0.0548        & 0.0992        & 0.2988        \\ \hline
ToeSegmentation2               & 0.0718        & 0.144         & 0.3784        \\ \hline
Trace                          & 0.0222        & 0.0555        & 0.3752        \\ \hline
TwoLeadECG                     & 0.0045        & 0.0081        & 0.0259        \\ \hline
Two                            & 0.0038        & 0.0097        & 0.0259        \\ \hline
UWaveGestureLibraryAll         & 0.0025        & 0.0056        & 0.024         \\ \hline
uWaveGestureLibrary            & 0.0017        & 0.0024        & 0.0081        \\ \hline
wafer                          & 0.001         & 0.0032        & 0.0097        \\ \hline
Wine                           & 0.031         & 0.0477        & 0.1745        \\ \hline
WordsSynonyms                  & 0.0094        & 0.0196        & 0.0389        \\ \hline
Worms                          & 0.0661        & 0.109         & 0.3177        \\ \hline
WormsTwoClass                  & 0.0575        & 0.1193        & 0.3289        \\ \hline
yoga                           & 0.0017        & 0.0028        & 0.0096        \\ \hline
\end{tabular}
\label{tab:sampling}
\end{table}

\begin{table}[H]
\centering
\caption{Output dimension required for target $TLB$ across dimensionality reduction technique.}
\label{tab:baseK}
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|l}
\cline{1-10}
\textbf{}                      & \multicolumn{3}{c|}{\textbf{TLB: 0.75}}    & \multicolumn{3}{c|}{\textbf{TLB: 0.90}}    & \multicolumn{3}{c|}{\textbf{TLB: 0.99}}    & \textbf{} \\ \cline{1-10}
\textbf{Dataset}               & \textit{PAA} & \textit{FFT} & \textit{PCA} & \textit{PAA} & \textit{FFT} & \textit{PCA} & \textit{PAA} & \textit{FFT} & \textit{PCA} & \textit{} \\ \cline{1-10}
50words                        & 9            & 9            & 7            & 18           & 14           & 10           & 62           & 28           & 25           &           \\ \cline{1-10}
Adiac                          & 7            & 8            & 4            & 15           & 13           & 6            & 69           & 34           & 20           &           \\ \cline{1-10}
ArrowHead                      & 9            & 9            & 4            & 16           & 13           & 8            & 73           & 33           & 26           &           \\ \cline{1-10}
Beef                           & 7            & 15           & 2            & 20           & 18           & 3            & 89           & 48           & 7            &           \\ \cline{1-10}
BeetleFly                      & 16           & 16           & 6            & 28           & 21           & 12           & 99           & 34           & 22           &           \\ \cline{1-10}
BirdChicken                    & 8            & 14           & 3            & 14           & 17           & 6            & 48           & 20           & 15           &           \\ \cline{1-10}
Car                            & 7            & 16           & 2            & 15           & 19           & 6            & 70           & 37           & 24           &           \\ \cline{1-10}
CBF                            & 15           & 13           & 7            & 61           & 57           & 45           & 114          & 114          & 107          &           \\ \cline{1-10}
ChlorineConcentration          & 46           & 34           & 2            & 93           & 81           & 5            & 153          & 153          & 30           &           \\ \cline{1-10}
CinC                           & 29           & 44           & 26           & 58           & 53           & 40           & 241          & 107          & 48           &           \\ \cline{1-10}
Coffee                         & 14           & 17           & 3            & 46           & 37           & 6            & 225          & 158          & 38           &           \\ \cline{1-10}
Computers                      & 21           & 24           & 16           & 94           & 66           & 44           & 636          & 614          & 192          &           \\ \cline{1-10}
Cricket                        & 14           & 14           & 9            & 47           & 35           & 21           & 248          & 202          & 113          &           \\ \cline{1-10}
DiatomSizeReduction            & 7            & 11           & 7            & 11           & 13           & 10           & 87           & 55           & 21           &           \\ \cline{1-10}
DPOAgeGroup   & 12           & 12           & 2            & 27           & 17           & 6            & 66           & 60           & 36           &           \\ \cline{1-10}
DPOCorrect    & 12           & 12           & 2            & 26           & 16           & 7            & 66           & 57           & 32           &           \\ \cline{1-10}
DistalPhalanxTW                & 12           & 12           & 2            & 27           & 16           & 6            & 66           & 60           & 34           &           \\ \cline{1-10}
Earthquakes                    & 276          & 269          & 103          & 410          & 400          & 190          & 491          & 490          & 340          &           \\ \cline{1-10}
ECG200                         & 8            & 7            & 3            & 29           & 22           & 6            & 72           & 56           & 41           &           \\ \cline{1-10}
ECG5000                        & 14           & 14           & 3            & 30           & 24           & 7            & 115          & 88           & 31           &           \\ \cline{1-10}
ECGFiveDays                    & 31           & 28           & 2            & 53           & 40           & 5            & 111          & 65           & 13           &           \\ \cline{1-10}
ElectricDevices                & 36           & 36           & 27           & 62           & 57           & 49           & 78           & 79           & 74           &           \\ \cline{1-10}
FaceAll                        & 28           & 24           & 8            & 50           & 35           & 20           & 110          & 81           & 48           &           \\ \cline{1-10}
FaceFour                       & 36           & 31           & 5            & 67           & 43           & 12           & 277          & 228          & 61           &           \\ \cline{1-10}
FacesUCR                       & 28           & 24           & 9            & 48           & 34           & 22           & 109          & 53           & 49           &           \\ \cline{1-10}
FISH                           & 10           & 15           & 5            & 20           & 18           & 11           & 91           & 37           & 28           &           \\ \cline{1-10}
FordA                          & 63           & 47           & 16           & 98           & 61           & 35           & 297          & 106          & 82           &           \\ \cline{1-10}
FordB                          & 69           & 49           & 19           & 102          & 65           & 39           & 318          & 107          & 85           &           \\ \cline{1-10}
Gun                            & 5            & 6            & 3            & 11           & 9            & 5            & 56           & 24           & 14           &           \\ \cline{1-10}
Ham                            & 34           & 32           & 7            & 73           & 58           & 18           & 261          & 114          & 61           &           \\ \cline{1-10}
HandOutlines                   & 11           & 70           & 10           & 25           & 83           & 32           & 93           & 91           & 46           &           \\ \cline{1-10}
Haptics                        & 10           & 29           & 6            & 19           & 35           & 14           & 173          & 81           & 32           &           \\ \cline{1-10}
Herring                        & 10           & 15           & 3            & 25           & 18           & 8            & 111          & 63           & 39           &           \\ \cline{1-10}
InlineSkate                    & 7            & 49           & 7            & 15           & 58           & 17           & 55           & 63           & 22           &           \\ \cline{1-10}
InsectWingbeatSound            & 15           & 14           & 7            & 28           & 22           & 13           & 100          & 42           & 33           &           \\ \cline{1-10}
ItalyPowerDemand               & 6            & 6            & 2            & 11           & 10           & 5            & 19           & 17           & 15           &           \\ \cline{1-10}
LargeKitchenAppliances         & 59           & 49           & 36           & 165          & 125          & 89           & 624          & 545          & 284          &           \\ \cline{1-10}
Lighting2                      & 41           & 34           & 9            & 152          & 149          & 28           & 557          & 490          & 82           &           \\ \cline{1-10}
Lighting7                      & 31           & 27           & 9            & 126          & 118          & 26           & 280          & 269          & 81           &           \\ \cline{1-10}
MALLAT                         & 19           & 30           & 10           & 46           & 36           & 26           & 297          & 182          & 36           &           \\ \cline{1-10}
Meat                           & 13           & 14           & 2            & 32           & 24           & 4            & 218          & 213          & 23           &           \\ \cline{1-10}
MedicalImages                  & 12           & 10           & 3            & 20           & 17           & 7            & 66           & 34           & 17           &           \\ \cline{1-10}
MPOAgeGroup   & 12           & 12           & 2            & 27           & 16           & 4            & 66           & 60           & 31           &           \\ \cline{1-10}
MPOCorrect    & 12           & 12           & 2            & 27           & 16           & 5            & 66           & 58           & 30           &           \\ \cline{1-10}
MiddlePhalanxTW                & 12           & 12           & 2            & 27           & 16           & 5            & 66           & 60           & 32           &           \\ \cline{1-10}
MoteStrain                     & 12           & 11           & 7            & 39           & 37           & 26           & 76           & 75           & 63           &           \\ \cline{1-10}
NonInvasiveFatalECG            & 16           & 22           & 3            & 42           & 31           & 18           & 201          & 121          & 82           &           \\ \cline{1-10}
OliveOil                       & 33           & 25           & 2            & 61           & 51           & 5            & 375          & 213          & 23           &           \\ \cline{1-10}
OSULeaf                        & 11           & 13           & 9            & 20           & 16           & 14           & 73           & 30           & 29           &           \\ \cline{1-10}
PhalangesOutlinesCorrect       & 11           & 12           & 2            & 26           & 16           & 5            & 65           & 56           & 28           &           \\ \cline{1-10}
Phoneme                        & 87           & 70           & 59           & 268          & 201          & 160          & 920          & 858          & 535          &           \\ \cline{1-10}
Plane                          & 12           & 11           & 3            & 22           & 14           & 6            & 76           & 39           & 21           &           \\ \cline{1-10}
PPOAgeGroup & 12           & 12           & 2            & 26           & 18           & 4            & 65           & 58           & 28           &           \\ \cline{1-10}
PPOCorrect  & 12           & 12           & 2            & 27           & 18           & 5            & 66           & 58           & 28           &           \\ \cline{1-10}
ProximalPhalanxTW              & 12           & 12           & 2            & 26           & 18           & 5            & 65           & 59           & 28           &           \\ \cline{1-10}
RefrigerationDevices           & 94           & 76           & 60           & 222          & 154          & 121          & 645          & 586          & 316          &           \\ \cline{1-10}
ScreenType                     & 18           & 24           & 20           & 70           & 55           & 40           & 614          & 614          & 207          &           \\ \cline{1-10}
ShapeletSim                    & 275          & 272          & 62           & 410          & 402          & 111          & 491          & 490          & 180          &           \\ \cline{1-10}
ShapesAll                      & 7            & 14           & 7            & 14           & 17           & 14           & 49           & 25           & 20           &           \\ \cline{1-10}
SmallKitchenAppliances         & 259          & 235          & 104          & 497          & 423          & 204          & 698          & 678          & 398          &           \\ \cline{1-10}
SonyAIBORobotSurface           & 15           & 14           & 5            & 28           & 21           & 13           & 56           & 43           & 38           &           \\ \cline{1-10}
SonyAIBORobotSurfaceII         & 18           & 18           & 6            & 30           & 24           & 13           & 57           & 45           & 39           &           \\ \cline{1-10}
StarLightCurves                & 5            & 27           & 2            & 14           & 33           & 21           & 51           & 36           & 35           &           \\ \cline{1-10}
Strawberry                     & 10           & 11           & 2            & 24           & 21           & 6            & 98           & 41           & 13           &           \\ \cline{1-10}
SwedishLeaf                    & 9            & 9            & 5            & 19           & 14           & 10           & 71           & 37           & 32           &           \\ \cline{1-10}
Symbols                        & 7            & 11           & 6            & 12           & 13           & 11           & 46           & 26           & 14           &           \\ \cline{1-10}
synthetic                      & 14           & 14           & 7            & 37           & 38           & 28           & 58           & 59           & 54           &           \\ \cline{1-10}
ToeSegmentation1               & 12           & 10           & 8            & 24           & 19           & 16           & 116          & 49           & 43           &           \\ \cline{1-10}
ToeSegmentation2               & 10           & 13           & 6            & 21           & 20           & 13           & 101          & 49           & 34           &           \\ \cline{1-10}
Trace                          & 6            & 9            & 2            & 18           & 17           & 7            & 120          & 69           & 31           &           \\ \cline{1-10}
TwoLeadECG                     & 12           & 9            & 2            & 25           & 19           & 4            & 70           & 51           & 14           &           \\ \cline{1-10}
Two                            & 13           & 11           & 7            & 34           & 24           & 20           & 108          & 102          & 98           &           \\ \cline{1-10}
UWGLAll         & 15           & 27           & 18           & 35           & 32           & 28           & 151          & 82           & 59           &           \\ \cline{1-10}
uWaveGestureLibrary            & 4            & 10           & 5            & 10           & 11           & 10           & 43           & 27           & 20           &           \\ \cline{1-10}
wafer                          & 12           & 10           & 4            & 37           & 29           & 11           & 125          & 112          & 49           &           \\ \cline{1-10}
Wine                           & 10           & 9            & 2            & 27           & 20           & 3            & 104          & 58           & 9            &           \\ \cline{1-10}
WordsSynonyms                  & 9            & 9            & 7            & 17           & 14           & 10           & 62           & 31           & 25           &           \\ \cline{1-10}
Worms                          & 9            & 26           & 8            & 26           & 30           & 17           & 123          & 62           & 41           &           \\ \cline{1-10}
WormsTwoClass                  & 10           & 26           & 8            & 25           & 30           & 17           & 124          & 61           & 42           &           \\ \cline{1-10}
yoga                           & 6            & 13           & 3            & 11           & 15           & 11           & 44           & 21           & 16           &           \\ \cline{1-10}
\end{tabular}
\end{table} 



\section{Additional End-to-End Lesion Plots}
\begin{figure}[H]
     \includegraphics[width=\linewidth]{figs/yoga.pdf} 
     \caption[]{yoga}
     \end{figure} 
     

 \begin{figure}[H]
     \includegraphics[width=\linewidth]{figs/uWaveGestureLibrary_Y.pdf} 
     \caption[]{uWaveGestureLibrary Y}
     \end{figure} 
     

 \begin{figure}[H] 
     \includegraphics[width=\linewidth]{figs/uWaveGestureLibrary_X.pdf} 
     \caption[]{uWaveGestureLibrary X}
     \end{figure} 
     

 \begin{figure}[H] 
     \includegraphics[width=\linewidth]{figs/uWaveGestureLibrary_Z.pdf} 
     \caption[]{uWaveGestureLibrary Z}
     \end{figure} 
     

 \begin{figure}[H] 
     \includegraphics[width=\linewidth]{figs/ElectricDevices.pdf} 
     \caption[]{ElectricDevices}
     \end{figure} 
 
     

 \begin{figure}[H] 
     \includegraphics[width=\linewidth]{figs/FordB.pdf} 
     \caption[]{FordB}
     \end{figure} 
     

 \begin{figure}[H] 
     \includegraphics[width=\linewidth]{figs/MALLAT.pdf} 
     \caption[]{MALLAT}
     \end{figure} 
     

 \begin{figure}[H] 
     \includegraphics[width=\linewidth]{figs/FordA.pdf} 
     \caption[]{FordA}
     \end{figure} 
     

 \begin{figure}[H] 
     \includegraphics[width=\linewidth]{figs/NonInvasiveFatalECG_Thorax1.pdf} 
     \caption[]{NonInvasiveFatalECG Thorax1}
     \end{figure} 
     

 \begin{figure}[H] 
     \includegraphics[width=\linewidth]{figs/NonInvasiveFatalECG_Thorax2.pdf} 
     \caption[]{NonInvasiveFatalECG Thorax2}
     \end{figure} 
     

 \begin{figure}[H] 
     \includegraphics[width=\linewidth]{figs/UWaveGestureLibraryAll.pdf} 
     \caption[]{UWaveGestureLibraryAll}
     \end{figure} 
     

 \begin{figure}[H] 
      \includegraphics[width=\linewidth]{figs/StarLightCurves.pdf} 
     \caption[]{StarLightCurves}
     \end{figure} 
\end{comment}



%\input{endendplots}


==> conclusion.tex <==

\begin{comment}
\begin{figure}
\includegraphics[width=\linewidth]{figs/beyond_tss_lesion.pdf}
\caption[]{End-to-End runtime lesion study of the entire MNIST dataset and the FMA featurized music dataset. Each of DROP's contributions provides a runtime improvement.}
\label{fig:beyond_lesion}
\end{figure}
\end{comment}



\section{Conclusion}
\label{sec:conclusion}

Advanced data analytics techniques must scale to rising data volumes. 
DR techniques offer a powerful toolkit when processing these datasets, with PCA frequently outperforming popular techniques in exchange for high computational cost. 
In response, we propose DROP, a new dimensionality reduction optimizer. 
DROP combines progressive sampling, progress estimation, and online aggregation to identify high quality low dimensional bases via PCA without processing the entire dataset by balancing the runtime of downstream tasks and achieved dimensionality. 
Thus, DROP provides a first step in bridging the gap between quality and efficiency in end-to-end DR for downstream \red{analytics}. 

%We revisit canonical operators for time series dimensionality reduction and the measurement study of~\cite{keogh-study}, and show that PCA is more effective than popular alternatives in the data mining literature often by a margin of over $2\times$ on average on gold-standard time series benchmark data sets with respect to output data dimension. More surprisingly, we empirically demonstrate that a small number of samples are sufficient to accurately characterize directions of maximum variance and obtain a high-quality low-dimensional transformation.




==> sampling.tex <==
\section{Sample-Based PCA}
\label{sec:sampling}

To tackle workload-aware DR, we demonstrate how sample-based PCA can bridge the performance , but that the number of samples required varies per dataset.
Finally, we show how dynamically increasing the sampling rate can help identify how much to sample a given dataset, providing a foundation for workload-aware DR.

\begin{figure}
\includegraphics[width=\linewidth]{figs/progressive.pdf}
\caption[]{ Improvement in representation size for  $TLB = 0.80$ across three datasets. Higher sampling rates improve quality until reaching a state equivalent to running PCA over the full dataset ("convergence")}
\label{fig:progressive}
\end{figure}

\begin{comment}
\subsection{PCA Speed vs. Quality}

While improved quality provides faster repeated query execution, the cost of DR via PCA dominates this speedup, encouraging the use of faster, lower-quality alternatives~\cite{keogh-study}. 

To briefly quantify this trade-off, we augment a widely-cited time series similarity search DR study from VLDB 2008~\cite{keogh-study} by evaluating PCA---which the authors did not benchmark due to it being ``untenable for large data sets." 
We compare PCA via SVD to baseline techniques based on runtime and DR performance with respect to $TLB$ over the largest datasets from~\cite{keogh-study}. 
We use their two fastest methods as our baselines as they show the remainder exhibited ``very little difference'': Fast Fourier Transform (FFT) and Piecewise Aggregate Approximation (PAA).

\minihead{TLB Performance Comparison}
We compute the minimum dimensionality achieved by each technique subject to a $TLB$ constraint. 
On average, PCA provides bases that are $2.3\times$ (up to $3.9\times$) and $3.7\times$ (up to $26\times$)  smaller than PAA and FFT for $TLB = 0.75$, and $2.9\times$ (up to $8.3\times$) and $1.8\times$ (up to $5.1\times$) smaller for $TLB = 0.99$.
While the margin between PCA and alternatives is dataset-dependent, PCA almost always preserves $TLB$ with a lower dimensional representation.

%\section{Additional End-to-End Plots}
%\input{endendplots}

\minihead{Runtime Performance Comparison} 
PCA implemented via out-of-the-box SVD is on average over \red{$26\times$ (up to $56\times$)} slower than PAA and over \red{$4.6\times$ (up to $9.7\times$)} times slower than FFT when computing the smallest $TLB$-preserving basis.
%This substantiates the observation that classic PCA is incredibly slow compared to alternatives~\cite{keogh-study}. 

\end{comment}

\subsection{Incremental, Progressive Sampling}
To bridge this performance-runtime gap, we turn to data sampling. 
Many real-world \red{datasets} are intrinsically low-dimensional, as evidenced by their rapid falloff in their eigenvalue spectrum.
A data sample thus captures much of the dataset's ``interesting'' behavior, so fitting models over data samples generalize well. 
We verify this by varying the target $TLB$ and examining the minimum number of uniformly selected samples required to obtain a $TLB$-preserving transform with output dimension $k$ equal to input dimension $\dvar$.

On average, a sample of under $0.64\%$ $(\text{up to } 5.5\%)$ of the input is sufficient for $TLB = 0.75$, and under $4.2\%$ $(\text{up to } 38.6\%)$ is sufficient for $TLB=0.99$.  
If this sample rate is known, we obtain up to \red{$91\times$ speedup} compared to a na\"ive implementation of PCA via SVD---with no algorithmic improvement. 

However, this benefit is dataset-dependent, and unknown a priori.
We thus turn to progressive sampling (gradually increasing the sample size) to identify how large a sample suffices.
Figure~\ref{fig:progressive} shows how the dimensionality required to attain a given $TLB$ changes when we vary dataset and proportion of data sampled.
Increasing the number of samples provides lower dimensional transformations for the same quality.
However, this decrease in dimension plateaus as the number of samples increases.
Thus, while progressive sampling would allow us to tune the amount of time spent on DR, we must determine when the downstream value of decreased dimension is overpowered by the cost of additional DR---that is, whether to sample to convergence (evaluated in \S\ref{subsec:lesion}) or terminate early (e.g., at $0.3$ proportion of data sampled for SmallKitchenAppliances). 






